Persistent Memory Programming Abstractions in Context of Concurrent Applications

The advent of non-volatile memory (NVM) technologies like PCM, STT, memristors and Fe-RAM is believed to enhance the system performance by getting rid of the traditional memory hierarchy by reducing the gap between memory and storage. This memory technology is considered to have the performance like that of DRAM and persistence like that of disks. Thus, it would also provide significant performance benefits for big data applications by allowing in-memory processing of large data with the lowest latency to persistence. Leveraging the performance benefits of this memory-centric computing technology through traditional memory programming is not trivial and the challenges aggravate for parallel/concurrent applications. To this end, several programming abstractions have been proposed like NVthreads, Mnemosyne and intel's NVML. However, deciding upon a programming abstraction which is easier to program and at the same time ensures the consistency and balances various software and architectural trade-offs is openly debatable and active area of research for NVM community. We study the NVthreads, Mnemosyne and NVML libraries by building a concurrent and persistent set and open addressed hash-table data structure application. In this process, we explore and report various tradeoffs and hidden costs involved in building concurrent applications for persistence in terms of achieving efficiency, consistency and ease of programming with these NVM programming abstractions. Eventually, we evaluate the performance of the set and hash-table data structure applications. We observe that NVML is easiest to program with but is least efficient and Mnemosyne is most performance friendly but involves significant programming efforts to build concurrent and persistent applications.

==> macros.tex <==
% comment a region

\newcommand{\punt}[1]{}
\newcommand{\cmnt}[1]{}


% a word should not be broken across lines
\newcommand{\nosplit}{\linebreak}

% no hyphenation
\def\nohyphens{\hyphenpenalty=10000\exhyphenpenalty=10000}

% ~ character
\newcommand{\tilda}{\symbol{126}}

% useful mathematical symbols

\newcommand{\ang}[1]{\langle #1 \rangle}
\newcommand{\Ang}[1]{\Big\langle #1 \Big\rangle}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% keywords for pseudocode

%% various theorem environments
%% Commented out because they are already defined in llncs file %%
%% Decommented out because they are not defined in sigplan class %%

\newtheorem{theorem}{Theorem}
%\renewcommand{\thetheorem}{\arabic{theorem}}

\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{property}[theorem]{Property}

\newtheorem{definition}{Definition}

\newcounter{history}
\newcommand{\hist}[1]{\refstepcounter{history} {#1}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-----------------Theorem Notations Defined by Petr --------------------------------------------------------------------------------------------------------
%% Defined by Petr

\newtheorem{acknowledgement}[theorem]{Acknowledgement}
\newtheorem{observation}[theorem]{Observation}


%------------------------------------------------------------------------------------------------------------------------------

% various references
\newcommand{\chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\stref}[1]{step~\ref{step:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\insref}[1]{line~\ref{ins:#1}}
\newcommand{\corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\axmref}[1]{Proposition~\ref{axm:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\eqnref}[1]{Eqn(\ref{eq:#1})}
\newcommand{\eqvref}[1]{Equivalence~(\ref{eqv:#1})}
\newcommand{\ineqref}[1]{Inequality~(\ref{ineq:#1})}
%\newcommand{\invref}[1]{(\ref{inv:#1})}
\newcommand{\exref}[1]{Example~\ref{ex:#1}}
\newcommand{\propref}[1]{Property~\ref{prop:#1}}
\newcommand{\obsref}[1]{Observation~\ref{obs:#1}}
\newcommand{\asmref}[1]{Assumption~\ref{asm:#1}}
\newcommand{\thref}[1]{Thread~\ref{th:#1}}
\newcommand{\trnref}[1]{Transaction~\ref{trn:#1}}

%\newcommand{\lineref}[1]{Line~\ref{lin:#1}}

%\newcommand{\algoref}[1]{{\sf Algo$_{\ref{algo:#1}}$}}
\newcommand{\algoref}[1]{{Algo~\ref{algo:#1}}}
\newcommand{\subsecref}[1]{SubSection{\ref{subsec:#1}}}

\newcommand{\histref}[1]{\ref{hist:#1}}

\newcommand{\apnref}[1]{Appendix~\ref{apn:#1}}
\newcommand{\invref}[1]{Invariant~\ref{inv:#1}}

\newcommand{\Chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\Secref}[1]{Section~\ref{sec:#1}}
\newcommand{\Figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\Tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\Stref}[1]{Step~\ref{step:#1}}
\newcommand{\Thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\Lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\Corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\Axmref}[1]{Proposition~\ref{axm:#1}}
\newcommand{\Defref}[1]{Definition~\ref{def:#1}}
\newcommand{\Eqref}[1]{eq(\ref{eq:#1})}
\newcommand{\Eqvref}[1]{Equivalence~(\ref{eqv:#1})}
\newcommand{\Ineqref}[1]{Inequality~(\ref{ineq:#1})}
\newcommand{\Exref}[1]{Example~\ref{ex:#1}}
\newcommand{\Propref}[1]{Property~\ref{prop:#1}}
\newcommand{\Obsref}[1]{Observation~\ref{obs:#1}}
\newcommand{\Asmref}[1]{Assumption~\ref{asm:#1}}

\newcommand{\Lineref}[1]{Line~\ref{lin:#1}}
\newcommand{\Algoref}[1]{{\sf Algo$_{\ref{algo:#1}}$}}

\newcommand{\Apnref}[1]{Section~\ref{apn:#1}}
\newcommand{\Invref}[1]{Invariant~\ref{inv:#1}}
\newcommand{\Confref}[1]{Conflict~\ref{conf:#1}}




\newcommand{\theqed}{$\Box$}


\newcommand{\nsqed}{\hspace*{\fill} \theqed}


% Renews the footnote command
\renewcommand{\thefootnote}{\alph{footnote}}

\newcommand{\ignore}[1]{}

\newcommand{\myparagraph}[1]{\vspace{1mm}\noindent\textbf{#1}}


%------------------------------------------------------------------------------------------------------------------
% Definitions for Object STM paper
%------------------------------------------------------------------------------------------------------------------
%

\newcommand{\tobj} {transaction object}
\newcommand{\txns}[1] {txns(#1)}
\newcommand {\comm}[1] {committed(#1)}
\newcommand {\aborted}[1] {aborted(#1)}
\newcommand {\incomp}[1] {incomp(#1)}
\newcommand {\live}[1] {live(#1)}
\newcommand {\term}[1] {term(#1)}
\newcommand {\key}[1] {key(#1)}
\newcommand {\confevt}[1] {conf-event(#1)}
\newcommand {\confmth}[1] {conf-method(#1)}
\newcommand {\conf}[1] {conflict(#1)}
\newcommand {\termn}[1] {terminate(#1)}

\newcommand {\tcomp} {t-complete}
\newcommand {\tinc} {t-incomplete}

\newcommand{\ssch} {sub-history}
\newcommand{\sschs} {sub-histories}

\newcommand{\nseq} {non-sequential}
\newcommand{\tseq} {t-sequential}
\newcommand{\seq} {sequential}
\newcommand{\serial} {serial}
\newcommand{\serialc} {serial criterion}

\newcommand{\lastw} {lastWrite}
\newcommand{\lwrite}[2] {#2.lastWrite(#1)}
\newcommand{\vwrite} {valWrite}
\newcommand{\valw}[2] {#2.valWrite(#1)}
\newcommand{\lastup} {lastUpdt}
\newcommand{\lupdt}[2] {#2.lastUpdt(#1)}
\newcommand{\lseen}[2] {#2.lastSeen(#1)}

\newcommand{\mr} {MR}
\newcommand{\tr} {TR}

\newcommand{\valid} {valid}
\newcommand{\validity} {validity}
\newcommand{\legal} {legal}
\newcommand{\legality} {legality}

\newcommand{\op} {operation}
\newcommand{\mth} {method}
\newcommand{\rvmt} {rv-method}
\newcommand{\upmt} {upd-method}


\newcommand{\termop} {terminal operation}
\newcommand{\cc} {correctness-criterion}
\newcommand{\ccs} {correctness-criteria}
\newcommand{\gen}[1] {gen(#1)}

\newcommand{\inv} {inv}
\newcommand{\rsp} {rsp}
\newcommand{\rmw} {rmw}
\newcommand{\first}[1] {first(#1)}
\newcommand{\last}[1] {last(#1)}

\newcommand{\evts}[1] {evts(#1)}
\newcommand{\met}[1] {methods(#1)}

\newcommand{\sgt} {SGT}
\newcommand{\memop} {memory operation}
\newcommand{\pref}[2] {#2.prefix(#1)}

%\newcommand{\begt} {begin\text{-}trans}
\cmnt{\newcommand{\tbeg} {\emph{t\_begin}}
\newcommand{\tread} {\emph{t\_read}}
\newcommand{\twrite} {\emph{t\_write}}
\newcommand{\tins} {\emph{t\_ins}}
\newcommand{\tdel} {\emph{t\_del}}
\newcommand{\tlook} {\emph{t\_look}}
\newcommand{\tryc} {\emph{tryCommit}}%{\emph{tryC}}
\newcommand{\trya} {\emph{tryA}}%{\emph{tryA}}
}

\newcommand{\tbeg} {\emph{begin}}
\newcommand{\tread} {\emph{read}}
\newcommand{\twrite} {\emph{write}}
\newcommand{\tins} {\emph{insert}}
\newcommand{\tdel} {\emph{delete}}
\newcommand{\tlook} {\emph{lookup}}
\newcommand{\tryc} {\emph{tryCommit}}%{\emph{tryC}}
\newcommand{\trya} {\emph{tryAbort}}%{\emph{tryA}}


\newcommand{\failed} {failed}
\newcommand{\unaborted} {unaborted}

\newcommand{\ins} {\emph{lsl\_insert}}
\newcommand{\del} {\emph{lsl\_del}}
\newcommand{\look} {\emph{lsl\_lookup}}
\newcommand{\lexec} {\emph{local execution}}
\newcommand{\valc} {\emph{validation-commit}}

\newcommand{\rv} {\emph{rv}}
\newcommand{\up} {\emph{up}}

\newcommand{\rset}[1] {rset(#1)}
\newcommand{\wset}[1] {wset(#1)}
\newcommand{\rvar} {readVar}

\newcommand{\co} {CO}
\newcommand{\opq} {opaque}
\newcommand{\opty} {opacity}
\newcommand{\coop} {co-opaque}
\newcommand{\coopty} {co\text{-}opacity}

\newcommand{\vwc} {VWC}
\newcommand{\lo} {LO}
\newcommand{\lopty} {LO}
\newcommand{\lopq} {locally-opaque}

\newcommand{\tab} {\texttt{hash-table}}
\newcommand{\set}{table}
\newcommand{\llist} {linked-list}
\newcommand{\otm} {\textit{OSTMs}}%{ObjSTM}
\newcommand{\rwtm} {\textit{RWSTMs}}
\newcommand{\lotm} {Table-OSTMs}
\newcommand{\bto} {BTO}

\newcommand{\csr} {CSR}

\newcommand{\perm} {permissive}
\newcommand{\pness} {permissiveness}
\newcommand{\permfn}[1] {perm(#1)}

\newcommand{\sspec} {sequential-specification}
\newcommand{\samp} {sample-stm}

\newcommand{\cg}[1] {CG(#1)}


\newcommand{\uset} {updtSet}
\newcommand{\lset} {lookupSet}
\newcommand{\rvm} {\emph{rvm}\xspace}


\newcommand{\firste} {firstEvt\xspace}
\newcommand{\laste} {lastEvt\xspace}
\newcommand{\fevt}[1] {#1.firstEvt}
\newcommand{\levt}[1] {#1.lastEvt}

\newcommand{\fkmth}[3] {#3.firstKeyMth(#1, #2)}
\newcommand{\pkmth}[3] {#3.prevKeyMth(#1, #2)}

\newcommand{\bstu} {\emph{bst-update}}
\newcommand{\lllist} {locallog\_list}

\newcommand{\udset}[1] {updtSet(#1)}
\newcommand{\rvset}[1] {rvSet(#1)}
\newcommand{\bst}{BST}
\newcommand{\lsl}{\emph{lazy-skip list}}

\newcommand{\refr}[1]{refNode(#1)}
\newcommand{\lin}[1]{#1.LP\xspace}

\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}%

\newcommand\tabspace[1][1cm]{\hspace*{#1}}

%%%%%%% DS macros
\newcommand{\glslhead}{getLslHead($obj\_id \downarrow, key \downarrow$)}
\newcommand{\llgopn}[1] {ll.getOpn($obj\_id \downarrow$, $ key \downarrow$)}
\newcommand{\llsopn}[1] {ll.setOpn(($obj\_id \downarrow$, $key \downarrow$, #1)}

\newcommand{\llgval}[1] {ll.getValue($obj\_id \downarrow$, $ key \downarrow$)}
\newcommand{\llsval}[1] {ll.setValue($obj\_id \downarrow$, $ key \downarrow$, #1)}

\newcommand{\llspc} {ll.setPreds\&Currs($obj\_id \downarrow$, $ key \downarrow$, $preds[] \downarrow$, $currs[] \downarrow$)}

\newcommand{\llgaptc}[1] {ll.getAptCurr(#1)}
\newcommand{\llgkeyobj} {ll.getKey\&Objid($ll\_entry_i \downarrow$)}

\newcommand{\llgopst} {ll.getOpStatus($obj\_id \downarrow$, $key \downarrow$)}
\newcommand{\llsopst}[1] {ll.setOpStatus($obj\_id \downarrow$, $ key \downarrow$, #1)}

\newcommand{\llgallpc}{ll.getAllPreds\&Currs($ll\_entry_i \downarrow$, $preds[] \uparrow$, $currs[] \uparrow$ )}

\newcommand{\poval}{poValidation($ll\_entry_i \downarrow$, $preds[] \uparrow$, $currs[] \uparrow$ )}


\newcommand{\txlfind} {\textup{txlog.findInLL}$(obj\_id \downarrow, key \downarrow)$}
\newcommand{\txgid} {txlog.getTid()}
\newcommand{\txgllist} {txlog.getLlList($t_{i} \downarrow$)}
\newcommand{\txsetst}[1] {txlog.setStatus($txstatus \downarrow$, $ OK \downarrow$)}
\newcommand{\txbegin}[1] {begin(#1)}

\newcommand{\lsls}[1] {lslSearch($obj\_id \downarrow$, $ key \downarrow$, $preds[] \uparrow$, $currs[] \uparrow$, $value_{BL} \uparrow$, #1)}

\newcommand{\rvvalidate} {rvValidate($ key \downarrow$, $preds[] \downarrow$, $currs[] \downarrow$)}

\newcommand{\lslins}[1] {lslIns($preds[] \downarrow$, $currs[] \downarrow$, #1)}
\newcommand{\lsldel} {lslDel($preds[] \downarrow$, $currs[] \downarrow$)}


\newcommand{\rlsol} {releaseOrderedLocks($ordered\_ll\_list \downarrow$)}

\newcommand{\ctov} {commitTOValidation($ll\_entry_i \downarrow$)}
\newcommand{\rvtov} {rvTOValidation($ key \downarrow$, $currs[] \downarrow$)}
\newcommand{\toval} {toValidation($ key \downarrow$, $currs[] \downarrow$, $val\_type \downarrow$)}
\newcommand{\validation} {validation($ key \downarrow$, $preds[] \downarrow$, $currs[] \downarrow$, $val\_type \downarrow$)}


\newcommand{\ifvalidation} {$($\textup{interferenceValidation}$(preds[] \downarrow, currs[] \downarrow))$}
\newcommand{\handlea}{tryAbort($obj\_id \downarrow$)}
\newcommand{\llsort}{ll.sort ($ll\_list \downarrow$)}

%%---------------------macro w/o parameter

\newcommand{\npctov} {\emph{commitTOValidation()}}
\newcommand{\nptov} {\emph{TOValidation()}}
\newcommand{\nptc} {\emph{tryCommit}}
\newcommand{\npins} {\emph{insert()}}
\newcommand{\npdel} {\emph{delete()}}
\newcommand{\npluk} {\emph{lookup()}}
\newcommand{\nplsls} {\emph{lslSearch()}}
\newcommand{\nplsldel} {\emph{lslDel()}}
\newcommand{\nplslins} {\emph{lslIns()}}
\newcommand{\npbegin} {\emph{begin}}
\newcommand{\nppoval} {\emph{poValidation}}


\newcommand{\rn} {\textcolor{red}{rednext}}
\newcommand{\bn} {\textcolor{blue}{bluenext}}

\newcommand{\rc} {\textcolor{red}{currs[0]}}
\newcommand{\bc} {\textcolor{blue}{currs[1]}}
\newcommand{\bp} {\textcolor{blue}{preds[0]}}
\newcommand{\rp} {\textcolor{red}{preds[1]}}


